CodeMind: Evaluating Large Language Models for Code Reasoning

Large Language Models (LLMs) have been widely used to automate programming tasks. Their capabilities have been evaluated by assessing the quality of generated code through tests or proofs. The extent to which they can reason about code is a critical question revealing important insights about their true capabilities. This paper introduces CodeMind, a framework designed to gauge the code reasoning abilities of LLMs through the following explicit and implicit code reasoning tasks: Independent Execution Reasoning (IER), Specification Reasoning (SR) and Dynamic Semantics Reasoning (DSR). The first evaluates the abilities of LLMs to simulate the execution of given inputs to a code and predict the output (IER). The second assesses the abilities of LLMs to incorporate the simulation of test data in the specification into code generation (SR). Finally, CodeMind evaluates LLMs' abilities to understand overall code semantics only given a specific input/output (DSR). Our extensive evaluation of ten LLMs across four widely used benchmarks using CodeMind shows that LLMs, depending on their size and training strategy, can reason about some dynamic aspects of code. However, their performance drops for code with higher complexity, non-trivial logical and arithmetic operators, non-primitive types, and API calls. We show that these reasoning tasks evaluate LLMs differently, and a comprehensive evaluation of code reasoning requires them all. Finally, we show that the performance of LLMs in bug repair is not correlated with any of the code reasoning tasks, and except for advanced frontier models, other LLMs do not incorporate code reasoning when performing bug repair.

==> Listings/api.tex <==
% \begin{wrapfigure}[19]{l}{.45\textwidth}
\begin{lstlisting}[style=stylewithcommentPy]
def f(text, strip_chars):
    return text[::-1].strip(strip_chars)[::-1]
f('tcmfsmj', 'cfj')
@@Ground Truth:@@
output=|'tcmfsm'|
@@GPT-4-Turbo@@
Predicted output: |'mfsm'|
@@Analysis:@@
The function f takes two parameters: a string |'text'| |and| a 
string |'|strip_chars|'|. The function performs the following
operations:
1. It reverses the string |'text'|. For the |input| |'tcmfsmj'|,
reversing it results |in 'jmsfmct'|.
2. It then strips characters |from| both ends of the
|reversed| string that are found |in| |'|strip_chars|'|.
In this case, |'|strip_chars|'| contains |'|cfj|'|. From |'|jmsfmct|'|,
the |'j'| at the beginning |and| ~'c' at the end are stripped,~
~resulting in 'msfm'~.
3. Finally, it reverses the stripped string again.
Reversing |'|msfm|'| results |in| |'|mfsm|'|.Therefore, the output of
executing the function f on the inputs |'tcmfsmj'| |and| |'cfj'| 
|is| |'|mfsm|'|.
\end{lstlisting}
% \end{wrapfigure}

==> Listings/loop_body.tex <==
% \begin{wrapfigure}[19]{r}{.5\textwidth}
\begin{lstlisting}[style=stylewithcommentPy]
def greatest_common_divisor(a: int, b: int) -> int:
    while b:
        a, b = b, a % b
    return a
greatest_common_divisor(144, 60)
@@Ground Truth:@@
output=12
@@DeepSeek-Coder-Instruct-33b@@
Predicted output: 60
@@Analysis:@@
First Iteration:
- b != 0, so the loop continues;  ~a = 60, b = 144 % 60~
~= 144~.
- a |and| b are updated to b |and| a % b respectively. Now, a =
144, b = 60.
Second Iteration:
- b != 0, so the loop continues. a = 60, b = 144 % 60 = 0.
- a |and| b are updated to b |and| a % b respectively. Now, a 
= 0, b = 60.
The loop terminates because b |is| 0.
The function returns the value of |"a"|, which |is| now ~60~.

\end{lstlisting}
% \end{wrapfigure}

==> Listings/loop_iterable.tex <==
\begin{lstlisting}[style=stylewithcommentPy]
def by_length(arr):
    dic = { 1: "One", 2: "Two", 3: "Three", 4: "Four", 5: "Five", 6: "Six", 7: "Seven", 8: "Eight", 9: "Nine"}
    sorted_arr = sorted(arr, reverse=True)
    new_arr = []
    for var in sorted_arr:
        try: new_arr.append(dic[var])
        except: pass
    return new_arr
by_length([2, 1, 1, 4, 5, 8, 2, 3]) 
@@Ground Truth:@@
output=[|'Eight'|, |'Five'|, |'Four'|, |'Three'|, |'Two'|, |'Two'|, |'One'|, |'One'|]
@@SemCoder-S@@
Predicted output: [|'Two'|, |'One'|, |'One'|, |'Four'|, |'Five'|, |'Eight'|, |'Two'|, |'Three'|]
@@Analysis:@@
In the given example, the |input| |list| |is| [2, 1, 1, 4, 5, 8, 
2, 3]. After sorting the |list in| descending order, it 
becomes [8, 5, 4, 3, 2, 2, 1, 1]. The function then 
~iterates over the sorted list.~ For each integer |in| 
`sorted_arr`, it tries to get the corresponding word |from| the 
dictionary. ~The strings corresponding to the numbers 2, 1,~
~1, 4, 5, 8, 2, 3~ are |'Two', 'One', 'One', 'Four', 'Five'|, 
|'Eight', 'Two', 'Three'|, respectively. So the output |list|
|is| [|'Two', 'One', 'One', 'Four', 'Five', 'Eight', 'Two'|, 
|'Three'|]. 

\end{lstlisting}

==> Listings/multi_predicate.tex <==
% \begin{wrapfigure}[19]{l}{.45\textwidth}
\begin{lstlisting}[style=stylewithcommentPy]
def monotonic(l: list):
    if l == sorted(l) or l == sorted(l, reverse=True):
        return True
    return False
monotonic([1, 2, 4, 10])
@@Ground Truth:@@
output=True
@@StarCoder2-15b@@
Predicted output: False
@@Analysis:@@
The code defines a function monotonic that takes a |list| l 
as an argument. It checks |if| the |list| |is| |sorted| |in|
ascending |or| descending order using the |sorted()| function.
If the list |sorted| |in| either order, the function returns 
True. Otherwise, it returns False. The ~list [1, 2, 4, 10]~
~is not sorted in ascending order so `l==sorted(l)` is false.~ 
It |is not sorted in| descending order so 
|`l==sorted(l, reverse=True)`| |is| also false. so the first
condition |is not| met |and| the function returns ~False~.

\end{lstlisting}
% \end{wrapfigure}

==> Listings/operators.tex <==
\begin{lstlisting}[style=stylewithcommentPy]
class CombinationCalculator:
    def __init__(self, datas: List[str]):
        self.datas = datas
  
    def count_all(n: int) -> int:
        if n < 0 or n > 63:
            return False
        return (1 << n) - 1 if n != 63 else float("inf")  
CombinationCalculator.count_all(0)
@@Ground Truth:@@
output=0
@@StarCoder2-15b@@
Predicted output: -1
@@Analysis:@@
The purpose of CombinationCalculator.count_all |is| to 
calculate the number of combinations of avgiven size m
|from| a |set| of n elements. In this case, n = 0.
Inside the count_all() method, the n parameter |is| checked to be within the |range| of 0 to 63.
If it |is not|, the method returns False.
Since n = 0, the method continues to the |next| line.
The method returns (1 << n) - 1 |if| n != 63, which |is| 
~0 - 1 = -1.~
\end{lstlisting}

==> Listings/wrong_branch.tex <==
\begin{lstlisting}[style=stylewithcommentPy]
def bf(planet1, planet2):
    planet_names = ("Mercury", "Venus", "Earth", "Mars", "Jupiter", "Saturn", "Uranus", "Neptune")
    if planet1 not in planet_names or planet2 not in planet_names or planet1 == planet2:
        return ()
    planet1_index = planet_names.index(planet1)
    planet2_index = planet_names.index(planet2)
    if planet1_index < planet2_index:
        return (planet_names[planet1_index + 1: planet2_index])
    else:
        return (planet_names[planet2_index + 1 : planet1_index])

bf(|"Jupiter"|, |"Neptune"|) 
@@Ground Truth:@@
output=(|'Saturn'|, |'Uranus'|)
@@Gemini-1.5-Pro@@
Predicted output: ()
@@Analysis:@@
The function `bf` |is| called with ( planet1 = |"Jupiter"|,
planet2 = |"Neptune"| ).
The first condition |`|planet1 |not| |in| planet_names |or| planet2
|not in| planet_names |or| planet1 == planet2|`| ~is false~, since
|all| the planets are present |in| the |list|.
The condition~ `planet1 == planet2`~ |is|  ~false~, since planet1 
|and| planet2 are different.
The ~ `planet1 not in planet_names`~ |is| ~false~, since planet1 
|is| present |in the list|.
The condition `planet2 |not in| planet_names` |is| also ~false~, 
since planet2 |is| present |in| the |list|.
Thus, ~the if branch is taken |and| the method returns ().~
\end{lstlisting}
